AASIST: Audio Anti-Spoofing using Integrated Spectro-Temporal Graph Attention Networks

Artefacts that differentiate spoofed from bona-fide utterances can reside in spectral or temporal domains. Their reliable detection usually depends upon computationally demanding ensemble systems where each subsystem is tuned to some specific artefacts. We seek to develop an efficient, single system that can detect a broad range of different spoofing attacks without score-level ensembles. We propose a novel heterogeneous stacking graph attention layer which models artefacts spanning heterogeneous temporal and spectral domains with a heterogeneous attention mechanism and a stack node. With a new max graph operation that involves a competitive mechanism and an extended readout scheme, our approach, named AASIST, outperforms the current state-of-the-art by 20% relative. Even a lightweight variant, AASIST-L, with only 85K parameters, outperforms all competing systems.

==> tables/table_smallBig.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYY}
    \Xhline{1pt}
	System & \# parameters & min t-DCF& EER	\\
    \Xhline{1pt}
	Li et al.~\cite{li2021channelwise} & 960K & N/R(0.0520) & N/R(1.78)\\
	\hline
	Hua et al.~\cite{hua2021towards}& 350K & N/R(0.0481) & N/R(1.64)\\
	\hline
	RawGAT-ST & 437K & 0.0443(0.0333) & 1.39(1.19)\\
	\hline
	Wang et al.~\cite{wang21fa_interspeech}&276K& N/R(0.0524) & N/R(1.92)\\
	\hline\hline
	AASIST & 297K & 0.0347(0.0275) & 1.13(0.83)\\
	\hline
	AASIST-L & 85K & 0.0362(0.0309) & 1.19(0.99)\\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	    Comparison on the number of parameters and performances, reported in ``average(best)'' after three repeated experiments.
	    A smaller variant, AASIST-L is reported (N/R: not reported). 
	}
% 	\vspace{-10pt}
	\label{tab:smallbig}
\end{table}

==> tables/table_sota_comparison.tex <==
\begin{table}[!t]
  \centering
  \begin{tabularx}{\columnwidth}{lcYY}
    \Xhline{1pt}
	System & Front-end & min t-DCF& EER	\\ 
    \Xhline{1pt}
	\textbf{AASIST} & Raw waveform & \textbf{0.0275} & \textbf{0.83}\\
	\hline
	 Tak et al.~\cite{tak2021end} & Raw waveform & 0.0335 & 1.06\\
	 \hline
	 Zhang et at.~\cite{zhang2021effect}&FFT&0.0368& 1.14\\
	 \hline
	 Hua et al.~\cite{hua2021towards}&Raw waveform&0.0481&1.64\\ 
	 \hline	
	 Ge et al.~\cite{ge2021raw}&Raw waveform&0.0517&1.77\\
	 \hline
	 Li et al.~\cite{li2021channelwise}&CQT&0.0520&1.78\\
	  \hline	
	 Chen et al.~\cite{chen2020generalization}&LFB&0.0520&1.81\\
	 \hline
	Wang et al.~\cite{wang21fa_interspeech}&LFCC&0.0524&1.92\\  
	 \hline	
	Luo et al.~\cite{luo2021capsule}&LFCC&0.0538&1.97\\  
	\hline
	Zhang et al.~\cite{zhang2021one}&LFCC&0.0590&2.19\\
	\hline
	Li et al.~\cite{li2021replay}&CQT&0.0743&2.50\\
	\hline
	Ma et al.~\cite{ma2021improved}&LFCC&0.0777&2.76\\
	\hline
	Tak et al.~\cite{tak2021graph}&LFB&0.0894&4.71\\
	\hline
    Tak et al.~\cite{tak2020spoofing}&LFCC&0.0904 &3.50\\
	\hline
	Ge et al.~\cite{ge2021}&LFCC&0.0914&4.96\\
% 	\hline
% 	Das et al.~\cite{das2021data}&DASC-CQT&0.0940&3.13\\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	    Comparison with recently proposed state-of-the-art systems, reported using pooled min t-DCF and EER (\%). 
	    Displayed in ascending order using min t-DCF. For the proposed AASIST, we report the best single result. 
	    All results are single model performance without any kind of score-level ensemble.
	}
% 	\vspace{-10pt}
	\label{tab:comparison}
\end{table}
